In Search of the Long-Tail: Systematic Generation of Long-Tail Inferential Knowledge via Logical Rule Guided Search

To effectively use large language models (LLMs) for real-world queries, it is imperative that they generalize to the long-tail distribution, i.e. rare examples where models exhibit low confidence. In this work, we take the first step towards evaluating LLMs in the long-tail distribution of inferential knowledge. We exemplify long-tail evaluation on the Natural Language Inference task. First, we introduce Logic-Induced-Knowledge-Search (LINK), a systematic long-tail data generation framework, to obtain factually-correct yet long-tail inferential statements. LINK uses variable-wise prompting grounded on symbolic rules to seek low-confidence statements while ensuring factual correctness. We then use LINK to curate Logic-Induced-Long-Tail (LINT), a large-scale long-tail inferential knowledge dataset that contains 108K statements spanning four domains. We evaluate popular LLMs on LINT; we find that state-of-the-art LLMs show significant performance drop (21% relative drop for GPT4) on long-tail data as compared to on head distribution data, and smaller models show even more generalization weakness. These results further underscore the necessity of long-tail evaluation in developing generalizable LLMs.

==> figures/evaluation.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{images/evaluation.pdf}
    \caption{Human evaluation of generation quality. \dataset has the higher plausibility accuracy and entailment accuracy than two large language model baselines. \todo{GPT4 fake numbers.}}
    \label{fig:evaluation}
\end{figure}



==> figures/p1_teaser.tex <==
\begin{figure*}[ht]
\vspace{-0.5cm}
    \centering
    \captionsetup{width=\textwidth}
    \includegraphics[width=\textwidth]{images/acl_teaser.pdf}
    \caption{
        An illustration of the distribution of statements generated by different methods, \ti{after being filtered on factual correctness by human evaluation}. For the same symbolic rule, all methods generate the same number of statements, but~\framework(\benchmarkEmoji) has more correct statements than zero-shot~\chat~and zero-shot~\gpt(\modelEmoji). ~\framework~\lt generations clearly lie in a more \lt part of the probability distribution than the zero-shot~\gpt~generations. \todo{add comparison to head distribution data}}
        \looseness=-1
        % \gpt~also made \todo{twice} as many factual errors in the bottom 20\% (40 statements) in the \lt distribution than \framework.
        % In the bottom 20\% (40 statements) of each model's distribution, \framework~only made 9 factual errors, while \gpt~made 18 factual errors.
        
        % We show 5 randomly sampled statements each from the bottom 20\% of \framework(\benchmarkEmoji) and \gpt(\modelEmoji)'s \lt distribution generation.
    \label{fig:teaser}
\end{figure*}

==> sections/7_statements.tex <==
\section*{Reproducibility statement}
\paragraph{Algorithm.} We provide accurate description of our \framework~framework in~\Secref{sec:link}, with additional details on creating symbolic rules in Appendix~\ref{app:rule_creation} and on critic model in Appendix~\ref{app:filter_job}. We include details of the entailment classification task in Appendix~\ref{app:probing_template}.

\paragraph{Prompt Engineering.} The prompts we used for conducting Knowledge Beam Search, generating \lt statements with LLMs and creating symbolic rules are described and exemplified in the main paper.

\paragraph{Data and Source Code.} The symbolic rules we use for \framework, all data generated by \framework, the human annotation data on \dataset~and the entailment classification task data are submitted with the paper. Data generated by ChatGPT and GPT4 as well as their human annotation will be available to the public upon request. Source code for creating symbolic rules, building \framework~and conducting entailment classification task will be released publicly after the anonymity period.

\paragraph{Crowdsourcing.} Templates for generation quality evaluation task and entailment classification task are included in Appendix~\ref{app:amt_template}. Annotator agreement statistics is included in Appendix~\ref{app:agreement}.

\section*{Ethics Statement}
\paragraph{Data.} All data we collected through LLMs in our work are released publicly for usage and have been duly scrutinized by the authors. Data for all human studies that we conduct are also publicly released with this work, with appropriate annotator anonymizations.

\paragraph{Crowdsourcing.} All our crowdworkers are from countries where English is the primary language and recruited from Amazon Mechanic Turk. For all our human studies, the task is set up in a manner that ensure that the annotators receive compensation that is above minimum wage (\$15/hour). Since we conduct extensive qualification tasks before annotations, crowdworkers that participate in the qualification are compensated more than minimum wage, given the time taken to read and understand task instructions and examples. Furthermore, we ensure that we correspond with crowdworkers over email to address their queries. Crowdworkers have also been given bonuses for providing feedback to the task, or consistently providing good-quality annotations.

\paragraph{Potential Use.} Our framework \framework~may only be used for generations that follow the ethics guideline of the community. Using \framework~on mal-intention-ed rules or searching for toxic and harmful values is a potential threat, but the authors strongly condemn doing so.

==> tables/evaluation_and_distribution.tex <==
\begin{minipage}{\linewidth}
      \centering
      \begin{minipage}{0.3 \linewidth}
          \begin{table}[H]
                \centering
                \small
                \begin{tabular}{cccc}
                \toprule
                  Accuracy & ChatGPT & GPT4 & LINK \\
                   \midrule
                     Plausibility & 86.43 & xx.xx & 99.17 \\
                     Entailment & 70.73 & xx.xx & 88.53 \\
                     Overall & 60.75 & xx.xx & 87.87 \\
                \bottomrule
                \end{tabular}
                \caption{Human evaluation of generation quality. \dataset~has the higher plausibility accuracy and entailment accuracy than two large language model baselines. \todo{GPT4 fake numbers.}}
                \label{tab:evaluation}
            \end{table}
      \end{minipage}
      \hspace{0.1\linewidth}
      \begin{minipage}{0.65\linewidth}
          \begin{figure}[H]
            \captionsetup{width=0.9\textwidth}
              \includegraphics[width=\linewidth]{images/distribution.png}
              \caption{Both ChatGPT and GPT4 generations in the \lt distribution overlap with their generations in the head distribution. In contrast, \dataset generations clearly land on the \lt distribution of InstructGPT.}
            \label{fig:distribution}
          \end{figure}
      \end{minipage}
\end{minipage}

==> tables/p2_probing.tex <==

% \begin{table}[t]
%     \centering
%      \small
%     \begin{tabular}{lccccccc}
%     \toprule
%       \multirow{2}{*}{} & \multicolumn{2}{c}{InstructGPT} & \multicolumn{2}{c}{ChatGPT} & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{\makecell[c]{Human \\Baseline}}\\
%        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%           & Zero-Shot & COT & Zero-Shot & COT & Zero-Shot & COT & \\
%           \midrule
%           \textbf{Head} & & & & & & & \\
%          \hspace{2mm}- Positive Template & 10.28 & 35.38 & 42.88 & 50.71 & 55.47 & 67.58 & -\\
%          \hspace{2mm}- Negative Template & 90.22 & 73.60 & 77.03 & 69.83 & 87.26 & 81.34 & -\\
%          \rowcolor{lightgray!60}[\dimexpr\tabcolsep+0.1pt\relax]
%          \ All               & 53.33 & 55.96 & 61.27 & 61.01 & 72.59 & 74.99 & 83.12\\
%          \midrule
%          \textbf{Longtail} & & & & & & & \\
%          \hspace{2mm}- Positive Template & 14.06 & 35.73 & 43.95 & 49.60 & 52.40 & 64.34 & - \\
%          \hspace{2mm}- Negative Template & 86.90 & 71.78 & 74.24 & 68.12 & 84.46 & 78.09 & - \\
%          \rowcolor{lightgray!60}[\dimexpr\tabcolsep+0.1pt\relax]
%          \ All               & 53.28 & 55.14 & 60.26 & 59.57 & 69.66 & 71.74 & 82.44\\
%     \bottomrule
%     \end{tabular}
%     \caption{Performance on the entailment classification task of three LLMs and human baseline decrease on the \lt distribution compared to the head distribution. LLMs also have a template bias towards negative templates -- when the target token is ``no", ``false" and ``wrong".}
%     \label{tab:probing}
% \end{table}

% \begin{table*}[t]
%     \centering
%      % \small
%      % \footnotesize
%      \scriptsize
%     \begin{tabular}{clccccccc}
%     \toprule
%       \multirow{2}{*}{Domain} & \multirow{2}{*}{Distribution} & \multicolumn{2}{c}{InstructGPT} & \multicolumn{2}{c}{ChatGPT} & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{\makecell[c]{Human \\Baseline}}\\
%        \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%          & & Zero-Shot & COT & Zero-Shot & COT & Zero-Shot & COT & \\
%           \midrule
%           % temporal
%          \multirow{8}{*}{Temporal} & \textbf{Head} & & & & & & & \\
%          & \hspace{2mm}- Positive Template & 12.12 & 47.96 & 45.28 & 59.83 & 79.43 & 87.03 & -\\
%          & \hspace{2mm}- Negative Template & 88.23 & 79.33 & 83.57 & 80.35 & 86.20 & 79.81 & -\\
%          & \cellcolor{lightgray!60}\ All & \cellcolor{lightgray!60} 53.10 & \cellcolor{lightgray!60} 64.85 & \cellcolor{lightgray!60} 65.90 & \cellcolor{lightgray!60} 70.88 & \cellcolor{lightgray!60} 83.07 & \cellcolor{lightgray!60} 83.14 & \cellcolor{lightgray!60} 84.69 \\
%          \cmidrule{2-9}
%          % \midrule
%          & \textbf{Longtail} & & & & & & & \\
%          & \hspace{2mm}- Positive Template & 16.56 & 47.01 & 44.29 & 58.72 & 77.41 & 81.99 & - \\
%          & \hspace{2mm}- Negative Template & 83.89 & 76.02 & 79.90 & 76.92 & 83.08 & 76.39 & - \\
%          & \cellcolor{lightgray!60}\ All & \cellcolor{lightgray!60} 52.81 & \cellcolor{lightgray!60} 62.63 & \cellcolor{lightgray!60} 63.46 & \cellcolor{lightgray!60} 68.52 & \cellcolor{lightgray!60} 80.46 & \cellcolor{lightgray!60} 78.97 & \cellcolor{lightgray!60} 83.20\\
%          \midrule
%          % food
%          \multirow{8}{*}{\makecell[c]{Capability and Advice}} & \textbf{Head} & & & & & & & \\
%          & \hspace{2mm}- Positive Template & 22.61 & 52.85 & 61.84 & 70.38 & 74.64 & 78.46 & -\\
%          & \hspace{2mm}- Negative Template & 84.80 & 71.65 & 77.66 & 74.91 & 86.93 & 84.63 & -\\
%          & \cellcolor{lightgray!60}\ All & \cellcolor{lightgray!60} 56.10 & \cellcolor{lightgray!60} 62.97 & \cellcolor{lightgray!60} 70.36 & \cellcolor{lightgray!60} 72.82 & \cellcolor{lightgray!60} 81.26 & \cellcolor{lightgray!60} 81.78 & \cellcolor{lightgray!60} 83.83\\
%          \cmidrule{2-9}
%          & \textbf{Longtail} & & & & & & & \\
%          & \hspace{2mm}- Positive Template & 27.66 & 55.38 & 67.01 & 68.77 & 72.87 & 80.89 & - \\
%          & \hspace{2mm}- Negative Template & 78.22 & 69.71 & 74.19 & 74.24 & 82.87 & 79.60 & - \\
%          & \cellcolor{lightgray!60}\ All & \cellcolor{lightgray!60} 54.88 & \cellcolor{lightgray!60} 63.09 & \cellcolor{lightgray!60} 70.88 & \cellcolor{lightgray!60} 71.71 & \cellcolor{lightgray!60} 78.25 & \cellcolor{lightgray!60} 80.19 & \cellcolor{lightgray!60} 85.13\\
%          \midrule
%          % natural
%          \multirow{8}{*}{\makecell[c]{Natural \\Properties}} & \textbf{Head} & & & & & & & \\
%          & \hspace{2mm}- Positive Template & 3.47 & 18.52 & 33.54 & 35.95 & 31.33 & 50.13 & -\\
%          & \hspace{2mm}- Negative Template & 93.85 & 70.75 & 72.68 & 60.96 & 89.05 & 81.58 & -\\
%          & \cellcolor{lightgray!60}\ All & \cellcolor{lightgray!60} 52.13 & \cellcolor{lightgray!60} 46.64 & \cellcolor{lightgray!60} 54.62 & \cellcolor{lightgray!60} 49.41 & \cellcolor{lightgray!60} 62.41 & \cellcolor{lightgray!60} 67.07 & \cellcolor{lightgray!60} 82.31\\
%          \cmidrule{2-9}
%          & \textbf{Longtail} & & & & & & & \\
%          & \hspace{2mm}- Positive Template & 3.71 & 16.97 & 33.39 & 34.09 & 24.62 & 44.53 & - \\
%          & \hspace{2mm}- Negative Template & 93.84 & 70.50 & 71.21 & 60.13 & 87.36 & 79.57 & - \\
%          & \cellcolor{lightgray!60}\ All & \cellcolor{lightgray!60} 52.24 & \cellcolor{lightgray!60} 45.79 & \cellcolor{lightgray!60} 53.75 & \cellcolor{lightgray!60} 48.11 & \cellcolor{lightgray!60} 58.40 & \cellcolor{lightgray!60} 63.40 & \cellcolor{lightgray!60} 82.45\\
%          \midrule
%          % locational
%          \multirow{8}{*}{Locational} & \textbf{Head} & & & & & & & \\
%          & \hspace{2mm}- Positive Template & 22.86 & 52.86 & 51.67 & 63.10 & 52.14 & 59.29 & -\\
%          & \hspace{2mm}- Negative Template & 87.55 & 65.92 & 68.98 & 61.84 & 75.71 & 77.14 & -\\
%          & \cellcolor{lightgray!60}\ All & \cellcolor{lightgray!60} 57.69 & \cellcolor{lightgray!60} 59.89 & \cellcolor{lightgray!60} 60.99 & \cellcolor{lightgray!60} 62.42 & \cellcolor{lightgray!60} 64.84 & \cellcolor{lightgray!60} 68.90 & \cellcolor{lightgray!60} 75.71\\
%          \cmidrule{2-9}
%          & \textbf{Longtail} & & & & & & & \\
%          & \hspace{2mm}- Positive Template & 41.39 & 57.30 & 51.87 & 57.68 & 59.74 & 63.30 & - \\
%          & \hspace{2mm}- Negative Template & 76.24 & 62.12 & 63.40 & 58.11 & 73.03 & 70.30 & - \\
%          & \cellcolor{lightgray!60}\ All & \cellcolor{lightgray!60} 60.16 & \cellcolor{lightgray!60} 59.90 & \cellcolor{lightgray!60} 58.08 & \cellcolor{lightgray!60} 57.91 & \cellcolor{lightgray!60} 66.90 & \cellcolor{lightgray!60} 67.07 & \cellcolor{lightgray!60} 67.42\\
%     \bottomrule
%     \end{tabular}
%     \caption{Performance on the entailment classification task of three LLMs and human baseline decrease on the \lt distribution compared to the head distribution. LLMs also have a template bias towards negative templates -- when the target token is ``no'', ``false'' and ``wrong''.}
%     \label{tab:probing}
% \end{table*}


\begin{table*}[t]
\vspace{-0.4cm}
    \centering
     % \small
     % \footnotesize
     \scriptsize
    \begin{tabular}{cclccccccc}
    \toprule
      \multirow{2}{*}{Domain} & \multirow{2}{*}{Distribution}  & \multirow{2}{*}{Template}& \multicolumn{2}{c}{InstructGPT} & \multicolumn{2}{c}{ChatGPT} & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{\makecell[c]{Human \\Baseline}}\\
       \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
         & & & Zero-Shot & COT & Zero-Shot & COT & Zero-Shot & COT & \\
          \midrule
          % natural
         \multirow{6}{*}{\makecell[c]{Natural \\Properties}} & \multirow{3}{*}{Head}
         & Positive Template & 3.47 & 18.52 & 33.54 & 35.95 & 31.33 & 50.13 & -\\
         & & Negative Template & 93.85 & 70.75 & 72.68 & 60.96 & 89.05 & 81.58 & -\\
         & & \cellcolor{lightgray!60}All & \cellcolor{lightgray!60} 52.13 & \cellcolor{lightgray!60} 46.64 & \cellcolor{lightgray!60} 54.62 & \cellcolor{lightgray!60} 49.41 & \cellcolor{lightgray!60} 62.41 & \cellcolor{lightgray!60} 67.07 & \cellcolor{lightgray!60} 82.31\\
         \cmidrule{2-10}
         & \multirow{3}{*}{Longtail}
         & Positive Template & 3.71 & 16.97 & 33.39 & 34.09 & 24.62 & 44.53 & - \\
         & & Negative Template & 93.84 & 70.50 & 71.21 & 60.13 & 87.36 & 79.57 & - \\
         & & \cellcolor{lightgray!60}All & \cellcolor{lightgray!60} 52.24 & \cellcolor{lightgray!60} 45.79 & \cellcolor{lightgray!60} 53.75 & \cellcolor{lightgray!60} 48.11 & \cellcolor{lightgray!60} 58.40 & \cellcolor{lightgray!60} 63.40 & \cellcolor{lightgray!60} 82.45\\
         \midrule
          % temporal
         \multirow{6}{*}{Temporal} & \multirow{3}{*}{Head}
         & Positive Template & 12.12 & 47.96 & 45.28 & 59.83 & 79.43 & 87.03 & -\\
         & & Negative Template & 88.23 & 79.33 & 83.57 & 80.35 & 86.20 & 79.81 & -\\
         & & \cellcolor{lightgray!60}All & \cellcolor{lightgray!60} 53.10 & \cellcolor{lightgray!60} 64.85 & \cellcolor{lightgray!60} 65.90 & \cellcolor{lightgray!60} 70.88 & \cellcolor{lightgray!60} 83.07 & \cellcolor{lightgray!60} 83.14 & \cellcolor{lightgray!60} 84.69 \\
         \cmidrule{2-10}
         % \midrule
         % & \textbf{Longtail} & & & & & & & \\
         & \multirow{3}{*}{Longtail} & Positive Template & 16.56 & 47.01 & 44.29 & 58.72 & 77.41 & 81.99 & - \\
         & & Negative Template & 83.89 & 76.02 & 79.90 & 76.92 & 83.08 & 76.39 & - \\
         & & \cellcolor{lightgray!60}All & \cellcolor{lightgray!60} 52.81 & \cellcolor{lightgray!60} 62.63 & \cellcolor{lightgray!60} 63.46 & \cellcolor{lightgray!60} 68.52 & \cellcolor{lightgray!60} 80.46 & \cellcolor{lightgray!60} 78.97 & \cellcolor{lightgray!60} 83.20\\
         \midrule
         % food
         \multirow{6}{*}{\makecell[c]{Capability \\ and Advice}} & \multirow{3}{*}{Head}
         & Positive Template & 22.61 & 52.85 & 61.84 & 70.38 & 74.64 & 78.46 & -\\
         & & Negative Template & 84.80 & 71.65 & 77.66 & 74.91 & 86.93 & 84.63 & -\\
         & & \cellcolor{lightgray!60}All & \cellcolor{lightgray!60} 56.10 & \cellcolor{lightgray!60} 62.97 & \cellcolor{lightgray!60} 70.36 & \cellcolor{lightgray!60} 72.82 & \cellcolor{lightgray!60} 81.26 & \cellcolor{lightgray!60} 81.78 & \cellcolor{lightgray!60} 83.83\\
         \cmidrule{2-10}
         & \multirow{3}{*}{Longtail}
         & Positive Template & 27.66 & 55.38 & 67.01 & 68.77 & 72.87 & 80.89 & - \\
         & & Negative Template & 78.22 & 69.71 & 74.19 & 74.24 & 82.87 & 79.60 & - \\
         & & \cellcolor{lightgray!60}All & \cellcolor{lightgray!60} 54.88 & \cellcolor{lightgray!60} 63.09 & \cellcolor{lightgray!60} 70.88 & \cellcolor{lightgray!60} 71.71 & \cellcolor{lightgray!60} 78.25 & \cellcolor{lightgray!60} 80.19 & \cellcolor{lightgray!60} 85.13\\
         \midrule
         % locational
         \multirow{6}{*}{Locational} & \multirow{3}{*}{Head}
         & Positive Template & 22.86 & 52.86 & 51.67 & 63.10 & 52.14 & 59.29 & -\\
         & & Negative Template & 87.55 & 65.92 & 68.98 & 61.84 & 75.71 & 77.14 & -\\
         & & \cellcolor{lightgray!60}All & \cellcolor{lightgray!60} 57.69 & \cellcolor{lightgray!60} 59.89 & \cellcolor{lightgray!60} 60.99 & \cellcolor{lightgray!60} 62.42 & \cellcolor{lightgray!60} 64.84 & \cellcolor{lightgray!60} 68.90 & \cellcolor{lightgray!60} 75.71\\
         \cmidrule{2-10}
         & \multirow{3}{*}{Longtail}
         & Positive Template & 41.39 & 57.30 & 51.87 & 57.68 & 59.74 & 63.30 & - \\
         & & Negative Template & 76.24 & 62.12 & 63.40 & 58.11 & 73.03 & 70.30 & - \\
         & & \cellcolor{lightgray!60}All & \cellcolor{lightgray!60} 60.16 & \cellcolor{lightgray!60} 59.90 & \cellcolor{lightgray!60} 58.08 & \cellcolor{lightgray!60} 57.91 & \cellcolor{lightgray!60} 66.90 & \cellcolor{lightgray!60} 67.07 & \cellcolor{lightgray!60} 67.42\\
    \bottomrule
    \end{tabular}
    \caption{Performance on the entailment classification task of three LLMs decreases on the \lt distribution compared to the head distribution, while human performance does not. LLMs also have a template bias towards negative templates -- when the target token is ``no'', ``false'' and ``wrong''.}
    \label{tab:probing}
\end{table*}
% this will eventually be a table

==> tables/separation_probing.tex <==
% \begin{wraptable}{r}{0.45 \columnwidth}
    \begin{table}[ht]
        \centering
        \small
        \caption{Performance on the entailment classification task of GPT4.}
        \begin{tabular}{ccc}
        \toprule
           & Zero-Shot & COT \\
           \midrule
           Head & 73.49 & 76.24 \\
           Longtail & 68.47 & 70.75\\
           $\Delta$ & -5.02\% & -5.49\%\\
        \bottomrule
        \end{tabular}
        \label{tab:sep_probing}
    \end{table}
% \end{wraptable}
